NL2Formula: Generating Spreadsheet Formulas from Natural Language Queries

Writing formulas on spreadsheets, such as Microsoft Excel and Google Sheets, is a widespread practice among users performing data analysis. However, crafting formulas on spreadsheets remains a tedious and error-prone task for many end-users, particularly when dealing with complex operations. To alleviate the burden associated with writing spreadsheet formulas, this paper introduces a novel benchmark task called NL2Formula, with the aim to generate executable formulas that are grounded on a spreadsheet table, given a Natural Language (NL) query as input. To accomplish this, we construct a comprehensive dataset consisting of 70,799 paired NL queries and corresponding spreadsheet formulas, covering 21,670 tables and 37 types of formula functions. We realize the NL2Formula task by providing a sequence-to-sequence baseline implementation called fCoder. Experimental results validate the effectiveness of fCoder, demonstrating its superior performance compared to the baseline models. Furthermore, we also compare fCoder with an initial GPT-3.5 model (i.e., text-davinci-003). Lastly, through in-depth error analysis, we identify potential challenges in the NL2Formula task and advocate for further investigation.

==> preamble.tex <==
\acmConference[ICSE 2024]{46th International Conference on Software Engineering}{April 2024}{Lisbon, Portugal}

%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\usepackage{longfbox}
% \usepackage[skins]{tcolorbox
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage[american]{babel}
\usepackage{microtype}
\usepackage{subcaption}
\usepackage[ruled,,linesnumbered ]{algorithm2e}
\usepackage[most]{tcolorbox}
\usepackage{balance} % used to balance the two columns in bibliography
\usepackage{enumitem} % e.g., \begin{itemize}[leftmargin=*] \item \textbf{A collection of code corpus with preprocessing scripts.} xxxxx \end{itemize}
% \usepackage{lipsum}
% \usepackage{appendix}
%\usepackage{minted}
%\usepackage[flushleft]{threeparttable}
%\usepackage{tabularx}
%\usepackage{booktabs}
%\usepackage{hyperref}
%\usepackage{listings}
%\usepackage{spverbatim}
%\usepackage{multicol}
%\usepackage{multirow}
\usepackage{color}
\usepackage{url}
\usepackage{arydshln}
\usepackage{bm}
\usepackage{multirow}
% ===========================================================================


%========================New commands added by Yao Wan========================

% \usepackage{syntax}
\usepackage[nounderscore]{syntax}
\usepackage{tcolorbox}
\tcbuselibrary{skins, breakable, theorems}
\usepackage{colortbl}
\usepackage{geometry}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\nlformula}{\textsc{NL2Formula \xspace}}%
\newcommand{\nlformulanospace}{\textsc{NL2Formula}}%
\newcommand{\model}{$f$\textsc{Coder \xspace}}%
\newcommand{\modelnospace}{$f$\textsc{Coder}}%

% \newcommand{\grammarlabel}[2]{\synt{#1}\hfill#2}

% $f$\textsc{Coder}
% ========================================================================

%========================For source code typesetting========================
%\usepackage{minted} 
%\definecolor{graybg}{rgb}{0.95,0.95,0.95}
%\definecolor{bg}{rgb}{0.95,0.95,0.95}
% ========================================================================

%================ Insert colored comments in the text===========================
\newcount\DraftStatus  % 0 suppresses notes to selves in text
\DraftStatus=1   % TODO: set to 0 for final version
%=================================================================

\definecolor{darkgreen}{rgb}{0,0.5,0} % Darkgreen
\definecolor{purple}{rgb}{1,0,1} % Purple
\definecolor{todocolor}{rgb}{0.9,0.1,0.1} % Yellow&Green
\definecolor{fixcolor}{rgb}{0.1,0.7,0.3} % Green
\definecolor{wycolor}{rgb}{0.9,0.1,0.1} % Red
\definecolor{hycolor}{rgb}{0.7,0.7,0.3} % Yellow&Green
%other colors include blue, red, purple, cyan, darkgreen, etc.

\newcommand{\nbc}[3]{\ifnum\DraftStatus=1
	{\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
	{\textcolor{#3}{\sf\small$\blacktriangleright$\emph{#2}$\blacktriangleleft$}}
\fi}

\newcommand{\draftnote}[2]{\ifnum\DraftStatus=1
	\marginpar{
		\tiny\raggedright
		\hbadness=10000
		\def\baselinestretch{0.8}
		\textcolor{#1}{\textsf{\hspace{0pt}#2}}}
\fi}
% add yourself here:
\newcommand{\yao}[1]{\nbc{Yao}{#1}{wycolor}}
\newcommand{\hy}[1]{\nbc{HY}{#1}{hycolor}}
\newcommand{\zqbi}[1]{\nbc{ZQ}{#1}{todocolor}}
\newcommand{\todo}[1]{\nbc{TODO}{#1}{todocolor}}
\newcommand{\hytt}[1]{\texttt{\hyphenchar\font=\defaulthyphenchar #1}}
\newcommand{\Yao}[1]{\draftnote{red}{[Yao: #1]}}

%=================================================================

\usepackage{makecell}

\usepackage{array}
% \definecolor{azure(colorwheel)}{rgb}{0.0, 0.5, 1.0}
\definecolor{sqlcolor}{rgb}{0.0, 0.5, 1.0} % blue
\definecolor{formulacolor}{rgb}{1, 0, 1.0} % blue
\definecolor{darkgreen}{rgb}{0,0.5,0} % Darkgreen
\definecolor{purple}{rgb}{1,0,1} % Purple
\definecolor{todocolor}{rgb}{0.9,0.1,0.1} % Yellow&Green
\definecolor{fixcolor}{rgb}{0.1,0.7,0.3} % Green
\definecolor{wycolor}{rgb}{0.9,0.1,0.1} % Red
\definecolor{hycolor}{rgb}{0.7,0.7,0.3} % Yellow&Green
%other colors include blue, red, purple, cyan, darkgreen, etc.
\definecolor{hdcolor}{rgb}{1, 0, 1.0} % 
%================ Formula colors ===========================
\definecolor{color02}{rgb}{0.61,0.00,0.93}
\definecolor{color04}{rgb}{0.29,0.29,0.36}
\definecolor{color05}{rgb}{0.01,0.08,0.33}
\definecolor{color06}{rgb}{0.35,0.00,0.02}
\definecolor{color07}{rgb}{0.31,0.35,0.75}
\definecolor{color08}{rgb}{0.42,0.42,0.36}
\definecolor{color09}{rgb}{0.00,0.05,0.21}
\definecolor{color10}{rgb}{0.30,0.47,0.29}
\definecolor{color11}{rgb}{0.41,0.30,0.30}
\definecolor{color12}{rgb}{0.25,0.29,0.61}

%================ End Formula colors ===========================

\settopmatter{printacmref=false} 
% \usepackage{newfloat}

% \usepackage{syntax}

% \DeclareFloatingEnvironment[
%   % the file extension for the file used to create the list:
%   fileext   = logr,% don't use log here!
%   % the heading for the list:
%   listname  = {List of Grammars},
%   % the name used in captions:
%   name      = Grammar,
%   % the default floating parameters if the environment is used
%   % without optional argument:
%   placement = htp
% ]{Grammar}

% \grammarindent=80pt

% \setlength{\grammarparsep}{4pt plus 1pt minus 1pt} % increase separation between rules

